Statistically Enhanced Learning: a feature engineering framework to boost (any) learning algorithms

Feature engineering is of critical importance in the field of Data Science. While any data scientist knows the importance of rigorously preparing data to obtain good performing models, only scarce literature formalizes its benefits. In this work, we will present the method of Statistically Enhanced Learning (SEL), a formalization framework of existing feature engineering and extraction tasks in Machine Learning (ML). The difference compared to classical ML consists in the fact that certain predictors are not directly observed but obtained as statistical estimators. Our goal is to study SEL, aiming to establish a formalized framework and illustrate its improved performance by means of simulations as well as applications on real life use cases.

==> images/tex/FormalizationTreeSELNoCite.tex <==
% Tikz source https://texample.net/tikz/examples/filesystem-tree/

\begin{forest}
    % forest preamble: determine layout and format of tree
    direction switch
    [\Large{\textbf{Statistically Enhanced Learning}}
        [\textbf{\textit{Images}}
            [\textit{Color histogram}]
            [\textit{Wavelets}]
            [\textit{Moments}]
            [\textit{Fourier transform}]
        ]
        [\textbf{\textit{Text}}
            [\textit{Bag of words}]
            [\textit{$n$-gram}]
            [\textit{Character count}]
            [\textit{\textbf{Embeddings}}
                [\textit{word2vec}]
                [\textit{TF-IDF}]
          ]
        ]
        [\textbf{\textit{Tabular}}
            [\textbf{\textit{Mismeasured variables}}
                [\textit{Fourier transform}]
                [\textit{Kernel decomposition}]
                [\textit{GIV / 2SLS}]
                % [\textit{Probabilistic Random Forest}]
        ]
        [\textbf{\textit{Unobserved variables}}
            [\textit{Proxy}]
            [\textit{MLE}]
        ]
        [\textbf{\textit{Sequential}}
            [\textit{Moments }]
            [\textit{Cumulants}]
            [\textit{Time Series model}]
            ]
        ]
    ]
\end{forest}
